Control of Connected and Automated Vehicles: State of the Art and Future Challenges

Autonomous driving technology pledges safety, convenience, and energy efficiency. Challenges include the unknown intentions of other road users: communication between vehicles and with the road infrastructure is a possible approach to enhance awareness and enable cooperation. Connected and automated vehicles (CAVs) have the potential to disrupt mobility, extending what is possible with driving automation and connectivity alone. Applications include real-time control and planning with increased awareness, routing with micro-scale traffic information, coordinated platooning using traffic signals information, eco-mobility on demand with guaranteed parking. This paper introduces a control and planning architecture for CAVs, and surveys the state of the art on each functional block therein; the main focus is on techniques to improve energy efficiency. We provide an overview of existing algorithms and their mutual interactions, we present promising optimization-based approaches to CAVs control and identify future challenges.

==> tikzlibrarypositioning-plus.code.tex <==
% This is the TikZ library positioning-plus
% Load with \usetikzlibrary{positioning-plus}
%
% This small library extends TikZ options like 'above', 'left' or 'below right'
% so that they can be used with an optional prefixed factor seperated by ':' (colon)
%
% The option 'left=.5:of somenode' will place
% a new node .5cm (default 'node distance' is '1cm and 1cm') left to (somenode).
% The option 'above right=.2 and .7:of someothernode' will place
% a new node .2cm above and .7cm right of (someothernode).
%
% Additional the options 'xshift*' and 'yshift*' add an additional shift
% as a factor of 'node distance'
% Inspired by http://tex.stackexchange.com/a/117610/16595

\usetikzlibrary{positioning}
\usetikzlibrary{fit}

\pgfdeclaregenericanchor{corner south east}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north east}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner south west}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north west}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}

\tikzset{corner above left/.code=\tikz@lib@place@handle@{#1}{corner south east}{-1}{1}{corner north west}{0.707106781}}
\tikzset{corner above right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{1}{corner north east}{0.707106781}}
\tikzset{corner below left/.code=\tikz@lib@place@handle@{#1}{corner north east}{-1}{-1}{corner south west}{0.707106781}}
\tikzset{corner below right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{-1}{corner south east}{0.707106781}}

\tikzset{corner north left/.code =\tikz@lib@place@handle@{#1}{corner north east}{-1}{0}{corner north west}{1}}
\tikzset{corner north right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{0}{corner north east}{1}}
\tikzset{corner south left/.code =\tikz@lib@place@handle@{#1}{corner south east}{-1}{0}{corner south west}{1}}
\tikzset{corner south right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{0}{corner south east}{1}}

\tikzset{corner west above/.code =\tikz@lib@place@handle@{#1}{corner south west}{0}{1}{corner north west}{1}}
\tikzset{corner west below/.code=\tikz@lib@place@handle@{#1}{corner north west}{0}{-1}{corner south west}{1}}
\tikzset{corner east above/.code =\tikz@lib@place@handle@{#1}{corner south east}{0}{1}{corner north east}{1}}
\tikzset{corner east below/.code=\tikz@lib@place@handle@{#1}{corner north east}{0}{-1}{corner south east}{1}}

\tikzset{north left/.code =\tikz@lib@place@handle@{#1}{north east}{-1}{0}{north west}{1}}
\tikzset{north right/.code=\tikz@lib@place@handle@{#1}{north west}{1}{0}{north east}{1}}
\tikzset{south left/.code =\tikz@lib@place@handle@{#1}{south east}{-1}{0}{south west}{1}}
\tikzset{south right/.code=\tikz@lib@place@handle@{#1}{south west}{1}{0}{south east}{1}}

\tikzset{west above/.code =\tikz@lib@place@handle@{#1}{south west}{0}{1}{north west}{1}}
\tikzset{west below/.code=\tikz@lib@place@handle@{#1}{north west}{0}{-1}{south west}{1}}
\tikzset{east above/.code =\tikz@lib@place@handle@{#1}{south east}{0}{1}{north east}{1}}
\tikzset{east below/.code=\tikz@lib@place@handle@{#1}{north east}{0}{-1}{south east}{1}}

\newif\ifqrr@tikz@lib@place@postransform
\tikzset{node distance transformation/.is if=qrr@tikz@lib@place@postransform}
\def\tikz@lib@place@handle@@#1#2#3#4{%
  \pgfutil@in@{of }{#1}%
  \ifpgfutil@in@%
    \tikz@lib@place@of#1\tikz@stop{#4}%
  \else%
    \edef\tikz@lib@place@nums{#1}%
  \fi%
  \ifx\tikz@lib@place@nums\pgfutil@empty%
    % Ok, nothing to do, we have set the anchor and we are happy...
  \else%
    \expandafter\tikz@lib@place@parse@nums\expandafter{\tikz@lib@place@nums}%
    \pgf@x=#2\pgf@x%
    \pgf@y=#3\pgf@y%
    \ifqrr@tikz@lib@place@postransform
      \pgf@pos@transform{\pgf@x}{\pgf@y}% change from original
    \fi
    \edef\tikz@lib@pos@call{\noexpand\pgftransformshift{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \fi%
}

\def\tikz@lib@place@handle@#1#2#3#4#5#6{%
  \pgfutil@in@{:}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@#1\tikz@stop
    \ifx\pgf@temp\pgfutil@empty
      \let\pgf@temp\tikz@node@distance
    \fi
    \pgfmathsetmacro\pgf@tempa{(\pgf@tempa)*#4}%
    \pgfmathsetmacro\pgf@tempb{(\pgf@tempb)*#3}%
    \edef\pgf@marshal{\noexpand\tikz@lib@place@handle@{\pgf@temp}{#2}{\pgf@tempb}{\pgf@tempa}{#5}{#6}}%
    \pgf@marshal
  \else
    \def\tikz@anchor{#2}%
    \let\tikz@do@auto@anchor=\relax%
    \edef\tikz@temp{#1}%
    \def\tikz@lib@place@single@factor{#6}%
    \expandafter\tikz@lib@place@handle@@\expandafter{\tikz@temp}{#3}{#4}{#5}%
  \fi
}
\def\tikz@lib@place@handle@qrr@#1:#2\tikz@stop{%
  \pgfutil@in@{and}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@@#1\tikz@stop
  \else
    \tikz@lib@place@handle@qrr@@#1and#1\tikz@stop
  \fi
  \def\pgf@temp{#2}%
}
\def\tikz@lib@place@handle@qrr@@#1and#2\tikz@stop{%
  \def\pgf@tempa{#1}%
  \def\pgf@tempb{#2}%
}
\def\qrr@xyshift@starred#1#2#3{
  \edef\tikz@marshal{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
  \tikz@marshal
  \ifpgfutil@in@
    \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
  \else
    \let#3\tikz@node@distance
  \fi
  \pgfmathparse{(#1)*#3}%
  \ifpgfmathunitsdeclared
    \if#2x%
      \pgftransformshift{\pgfqpoint{\pgfmathresult pt}{0pt}}%
    \else
      \pgftransformshift{\pgfqpoint{0pt}{\pgfmathresult pt}}%
    \fi
  \else
    \ifx#2x
      \pgf@process{\pgfqpointxy{\pgfmathresult}{0}}%
    \else
      \pgf@process{\pgfqpointxy{0}{\pgfmathresult}}%
    \fi
    \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi}
\tikzset{
  xshift*/.code=\qrr@xyshift@starred{#1}x\pgf@tempb,
  yshift*/.code=\qrr@xyshift@starred{#1}y\pgf@tempa,
}

\def\pgfutil@firstofmany#1#2\pgf@stop{#1}
\def\pgfutil@secondofmany#1#2\pgf@stop{#2}
\def\tikz@lib@place@of@#1#2#3{%
  \def\pgf@tempa{fit bounding box}%
  \edef\pgf@temp{\expandafter\pgfutil@firstofmany#2\pgf@stop}
  \if\pgf@temp(%
    \tikz@lib@place@fit@scan{#2}{0}%
  \else\if\pgf@temp|
      \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
    \else\ifx\pgf@temp\tikz@activebar
        \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
      \else\if\pgf@temp-
          \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{2}%
        \else\if\pgf@temp+
            \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{3}%
          \else
            \def\pgf@tempa{#2}%
          \fi
        \fi
      \fi
    \fi
  \fi
  \expandafter\tikz@scan@one@point\expandafter\tikz@lib@place@remember\expandafter(\pgf@tempa)%
  \iftikz@shapeborder%
    % Ok, this is relative to a border.
    \iftikz@lib@ignore@size%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{center}}%
      \def\tikz@anchor{center}%
    \else%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{#3}}%
    \fi%
  \fi%
  \edef\tikz@lib@place@nums{#1}%
}
\def\tikz@lib@place@fit@scan#1#2{
  \pgf@xb=-16000pt\relax%
  \pgf@xa=16000pt\relax%
  \pgf@yb=-16000pt\relax%
  \pgf@ya=16000pt\relax%
  \if\pgfutil@firstofmany#1\pgf@stop(%
    \tikz@lib@fit@scan#1\pgf@stop%
  \else
    \tikz@lib@fit@scan(#1)\pgf@stop
  \fi
  \ifdim\pgf@xa>\pgf@xa
    % shouldn't happen
  \else
     \expandafter\def\csname pgf@sh@ns@fit bounding box\endcsname{rectangle}%
     \expandafter\edef\csname pgf@sh@np@fit bounding box\endcsname{%
       \def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
       \def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
     }%
     \expandafter\def\csname pgf@sh@nt@fit bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
     \expandafter\def\csname pgf@sh@pi@fit bounding box\endcsname{\pgfpictureid}%
     \ifcase#2\relax
     \or % 1 = vertical
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})}}}%
       \pgf@marshal
     \or % 2 = horizontal
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \or % 3 = both directions
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})},minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \fi
  \fi
}
\tikzset{
  fit bounding box/.code={\tikz@lib@place@fit@scan{#1}{0}},
  span vertical/.code={\tikz@lib@place@fit@scan{#1}{1}},
  span horizontal/.code={\tikz@lib@place@fit@scan{#1}{2}},
  span/.code={\tikz@lib@place@fit@scan{#1}{3}}}

\pgfmathdeclarefunction{x_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempb}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
\pgfmathdeclarefunction{y_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempa}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
%\tikzdeclarecoordinatesystem{node distance}{%
%  \tikz@cs@nd#1\tikz@stop}
%\def\tikz@cs@nd#1,#2\tikz@stop{%
%  \def\qrr@xyshift@starred@action##1{\pgftransformshift{##1}}%
%  \qrr@xyshift@starred{#1}x\pgf@tempb
%  \qrr@xyshift@starred{#2}y\pgf@tempa}
\endinput
